Relating galaxies across different redshift to study galaxy evolution

We propose a general framework leveraging the halo-galaxy connection to link galaxies observed at different redshift in a statistical way, and use the link to infer the redshift evolution of the galaxy population. Our tests based on hydrodynamic simulations show that our method can accurately recover the stellar mass assembly histories up to $z\sim 3$ for present star-forming and quiescent galaxies down to $10^{10}h^{-1}M_{\odot}$. Applying the method to observational data shows that the stellar mass evolution of the main progenitors of galaxies depends strongly on the properties of descendants, such as stellar mass, halo mass, and star formation states. Galaxies hosted by low-mass groups/halos at the present time have since $z\sim 1.8$ grown their stellar mass $\sim 2.5$ times as fast as those hosted by massive clusters. This dependence on host halo mass becomes much weaker for descendant galaxies with similar star formation states. Star-forming galaxies grow about 2-4 times faster than their quiescent counterparts since $z\sim 1.8$. Both TNG and EAGLE simulations over-predict the progenitor stellar mass at $z>1$, particularly for low-mass descendants.

==> reply.tex <==
Dear Editor-in-chief,

Thank you for forwarding the referee's report on our revised submission.
We also thank the reviewer for further comments on our manuscript.

Our responses to the referee's comment is attached below. The modification of
the manuscript is highlighted in red.

Yours sincerely,
Kai Wang
On behalf of the co-authors

-----------------------------------------------------------------------

Our reply to the referee's comment.

We think that the referee might have misunderstood the description related to
rho(z) and the method in our paper. We make the following restatements to
dispel confusion.

1. As stated in Sec-2.1 and shown in Fig. 1, we first use the galaxy-halo
connection to populate galaxies in subhalos, and then use the connection
provided subhalo merger trees to infer the evolution of galaxy properties.

2. In Sec-2.2, we assign stellar mass to subhalos using the subhalo abundance
matching method. In this process, we introduce rho(z) to describe the
correlation of the deviation of the stellar mass from the mean stellar
mass-peak halo mass relation (i.e. of epsilon_z) at a given z with that at z=0.

3. In Sec-2.3, we assign star formation states to subhalos with the conditional
age distribution matching method. The star formation state of each subhalo is
determined by its z_starve, which only depends on the assembly history of a
subhalo and has nothing to do with rho(z). The definition of z_starve is
explicitly expressed in equation (10) and explained in its context.

As shown in Fig.A2, the model of rho(z) does not have a significant impact on
our results, and we do not think it necessary to discuss it in more detail.

We changed some wording in the manuscript, below equation (6) and below
equation (7), hopefully to make this clearer.

-----------------------------------------------------------------------
Reviewer's Comments:
Reviewer: 1

Comments to the Author
The authors have addressed my comments, but I still am not satisfies regarding
the discussion of the correlation coefficient. I kindly ask the authors to
address this in more detail, along the lines discussed below (I first
repeat my comment from my second referee report (>>>OLD COMMENT), followed
by the reply by the authors (>>>REPLY) and my new comment (>>>NEW COMMENT)


>>> OLD COMMENT:

This does not adequately address my comment. I still feel the authors
should add some discussion explicitely showing how results change
if the correlation relation is modified wrt eq 8 (i.e., when the
value of 0.83 is varied over some reasonable range).

The authors have written below eq. (8) "We note that our results are insensitive
to rho(z)". Do the authors mean that even if they were to set rho(z)=0 (i.e.
no cross correlation at all) the results don't change? I find this hard to
believe. In particular, won't you find zero dependence on the z=0 star formation
state if rho(z) = 0?

The authors need to show for a few cases how the results change depending
on what they assume for rho(z).

In App. A the authors state that rho(z) has a weak dependence on the
descendant stellar mass, and that they decide to ignore this dependence.
They authors should SHOW this dependence, as knowing how rho(z) depends
on descendant stellar mass is interesting in its own right!

Also: when testing against the EAGLE simulation, described in App B, do the
authors use the same rho(z), or do they derive a new rho(z) directly
from the EAGLE simulation? The authors should derive rho(z) from the
EAGLE simulation and compare the results to those for TNG. It is instructive
to know how uncertain/certain rho(z) actualy is, and the authors should
add some discussion about this.

>>> REPLY:

- We added Fig. A2 to show how stellar mass histories change with different
rho(z).

- Here we want to emphasize that the stellar mass histories are mainly driven
by the evolution of M_p of subhalos and the M_*-M_p relation at different
redshift. The change of rho(z) only affects the scatter of the stellar
mass-halo mass relation, which is a secondary effect.

- We updated Fig. A1 to include the dependence of rho(z) on descendant stellar
mass.

- We use the same rho(z) for TNG, EAGLE, and the observation for consistency.

- We emphasize again that we just want to use a reasonable rho(z) to avoid
unphysical fluctuations in individual stellar mass histories. This paper is not
intended to investigate how rho(z) depends on specific implementations of
different simulations.


>>> NEW COMMENT:

I appologize for being difficult, but I am still not satisfied with the answer.
Fig A1 just demonstrates that rho(z) has no impact on the AVERAGE stellar
mass histories as function of (z=0) halo mass. I understand that.
However, unless I'm badly mistaken, rho(z) controls the amount by which
the stellar mass histories of SF galaxies differ from those of quiescent
galaxies of the same z=0 stellar/halo mass. I suspect that if there is
NO correlation (i.e., rho(z)=0) then the curves for SF and quiescent
galaxies (as in Figs 3 and 10) will be identical, while a stronger
correlation results in a larger difference between the curves.

The new aspect of this paper is this splitting of SF and quiescent
galaxies, and in my view the introduction of a non-zero rho(z) is
CRUCIAL for this. Hence, this deserves/needs a more detailed discussion.

I kindly ask the authors to
1) assess/demonstrate how the splitting of mass histories between SF and Q galaxies
   depends on rho(z)
2) Fig A1 demonstrates a STRONG dependence on stellar mass (not a weak dependence,  as claimed in the text). It thus makes sense to develop a somewhat more elaborate, stellar mass dependent model for rho(z) and explore whether that improves the  results or not.

Finally, I don't understand why the authors are so reluctant to
investigate how rho(z) in TNG differs from that in the EAGLE simulations.
As I mentioned above, this inclusion of rho(z) is the only novel aspect
of this paper, and in my opinion the paper would be significantly stronger
and more impactful if they would discuss how robust rho(z) is among
different simulations.



